A Compositional Resilience Index for Computationally Efficient Safety Analysis of Interconnected Systems

Interconnected systems such as power systems and chemical processes are often required to satisfy safety properties in the presence of faults and attacks. Verifying safety of these systems, however, is computationally challenging due to nonlinear dynamics, high dimensionality, and combinatorial number of possible faults and attacks that can be incurred by the subsystems interconnected within the network. In this paper, we develop a compositional resilience index to verify safety properties of interconnected systems under faults and attacks. The resilience index is a tuple serving the following two purposes. First, it quantifies how a safety property is impacted when a subsystem is compromised by faults and attacks. Second, the resilience index characterizes the needed behavior of a subsystem during normal operations to ensure safety violations will not occur when future adverse events occur. We develop a set of sufficient conditions on the dynamics of each subsystem to satisfy its safety constraint, and leverage these conditions to formulate an optimization program to compute the resilience index. When multiple subsystems are interconnected and their resilience indices are given, we show that the safety constraints of the interconnected system can be efficiently verified by solving a system of linear inequalities. We demonstrate our developed resilience index using a numerical case study on chemical reactors connected in series.

==> prelim.tex <==
\section{Preliminary Background}

% A continuous function $\alpha:[0,a)\mapsto[0,\infty)$ belongs to class $\mathcal{K}$ if it is strictly increasing and $\alpha(0)=0$. 
A continuous function $\alpha:[-b,a)\mapsto(-\infty,\infty)$ belongs to extended class $\mathcal{K}$ if it is strictly increasing and $\alpha(0)=0$ for some $a,b>0$.
Linear functions $\alpha(x)=cx$ defined over $[-b,a)$ are extended class $\mathcal{K}$ functions, where $c>0$ is some coefficient.


Consider a continuous-time control-affine system 
\begin{equation}\label{eq:dynamic}
    \dot{x}=f(x)+g(x)u
\end{equation}
where $x\in\mathcal{X}\subseteq\mathbb{R}^n$ is the system state, $u\in\mathcal{U}\subseteq\mathbb{R}^p$ is the control input, $f:\mathcal{X}\rightarrow\mathbb{R}^n$, and $g:\mathcal{X}\rightarrow\mathbb{R}^{n\times p}$. 
Let $\mathcal{C}$ be a safety set defined as $\mathcal{C}=\{x\in\mathcal{X}:h(x)\geq0\}$, where $h:\mathcal{X}\rightarrow\mathbb{R}$ is a continuously differentiable function. We say system \eqref{eq:dynamic} is safe with respect to $\mathcal{C}$ if $x\in\mathcal{C}$ for all time $t\geq 0$.


Safety of a system following dynamics in Eqn. \eqref{eq:dynamic} can be verified by control barrier function (CBF)-based approaches \cite{ames2016control}.
The definition of CBF is given as follows
\begin{definition}[CBF \cite{ames2016control}]\label{def:CBF}
Consider a dynamical system \eqref{eq:dynamic} and a continuously differentiable function $h:\mathcal{X}\rightarrow\mathbb{R}$. If there exists a locally Lipschitz extended class $\mathcal{K}$ function $\alpha$ such that for all $x\in\mathcal{X}$ the following inequality holds
\begin{equation*}
    \sup_{u\in\mathcal{U}}\bigg\{\frac{\partial h(x)}{\partial x}f(x)+\frac{\partial h(x)}{\partial x}g(x)u
    +\alpha(h(x))\bigg\}\geq 0,
\end{equation*}
then function $h$ is a CBF.
\end{definition}
In this paper, we focus on the class of CBFs given as in Definition \ref{def:CBF}, which are also known as zeroing CBFs (ZCBFs).  
A sufficient condition for the safety guarantee can be derived using ZCBF as follows.
\begin{lemma}[\cite{ames2016control}]\label{lemma:CBF}
Given a dynamical system \eqref{eq:dynamic} and a safe set $\mathcal{C}$ defined by a continuously differentiable function $h:\mathcal{X}\rightarrow\mathbb{R}$, if $h$ is a ZCBF defined on $\mathcal{X}$, then $\mathcal{C}$ is forward invariant.
\end{lemma}

In the following, we present Farkas' Lemma which will be used to characterize the solvability of a finite set of linear inequalities.
\begin{lemma}[Farkas' Lemma \cite{fang1993linear}]\label{lemma:Farkas}
Let $A\in\mathbb{R}^{m\times n}$ and $b\in\mathbb{R}^m$. Then exactly one of the following two assertions is true:
\begin{enumerate}
    \item There exists an $x\in\mathbb{R}^n$ such that $Ax\leq b$ and $x\geq 0$.
    \item There exists a $y\in\mathbb{R}^m$ such that $A^\top y\geq 0$, $b^\top y<0$, and $y\geq 0$.
\end{enumerate}
\end{lemma}
